Effect of atomic interactions on quantum communication protocols

We develop a first-principles framework for analyzing photonic quantum communication in an atomic medium. Starting from a real-space quantization of the electromagnetic field coupled to an ensemble of two-level atoms, we derive an effective model for polarization-encoded single-photon states. We apply this framework to superdense coding to study communication efficiency and to the BB84 quantum key distribution protocol for communication security. For superdense coding, we evaluate the protocol capacity of the fixed Bell-state alphabet under erasure, dephasing, and depolarizing channels and show that it decreases monotonically with increasing atom-field coupling. For BB84, we formulate a modified protocol that discards erasure outcomes and uses the microscopic model to estimate the intrinsic loss rate. We derive the corresponding asymptotic key rate and show that it decreases monotonically with coupling strength and vanishes beyond a finite critical coupling.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
